On Generalized Bayesian Data Fusion with Complex Models in Large Scale Networks

Recent advances in communications, mobile computing, and artificial intelligence have greatly expanded the application space of intelligent distributed sensor networks. This in turn motivates the development of generalized Bayesian decentralized data fusion (DDF) algorithms for robust and efficient information sharing among autonomous agents using probabilistic belief models. However, DDF is significantly challenging to implement for general real-world applications requiring the use of dynamic/ad hoc network topologies and complex belief models, such as Gaussian mixtures or hybrid Bayesian networks. To tackle these issues, we first discuss some new key mathematical insights about exact DDF and conservative approximations to DDF. These insights are then used to develop novel generalized DDF algorithms for complex beliefs based on mixture pdfs and conditional factors. Numerical examples motivated by multi-robot target search demonstrate that our methods lead to significantly better fusion results, and thus have great potential to enhance distributed intelligent reasoning in sensor networks.

==> numexps.tex <==
%numexps
%...put results for numerical experiments here...
%\subsection{ISM vs. Other Approximations in Multiple Dims with Random GMs}
%...discuss results here -- need to do separate comparison between exact GM and WEP versions? Need to look at effect of pre-compression? 
%\subsection{Example Application: Outdoor Target Search}
...mainly to illustrate usefulness of hierarchical GM approximation with ISM method...can compare to non-hierarchical GM and to PF/WEM/FOCI/Chang-Sun approximation vs. exact grid fusion...thing to note here is that regions allow sensor likelihoods to be turned on/off as needed, e.g. agents in different regions pay attention to only updating GMs in those regions -- main takeaways: using ISM is more accurate within each region, and when fusion happens between agents, no need to look over or send every single mixand everywhere -- bandwidth/computation savings

